Lookahead: A Far-Sighted Alternative of Magnitude-based Pruning

Magnitude-based pruning is one of the simplest methods for pruning neural networks. Despite its simplicity, magnitude-based pruning and its variants demonstrated remarkable performances for pruning modern architectures. Based on the observation that magnitude-based pruning indeed minimizes the Frobenius distortion of a linear operator corresponding to a single layer, we develop a simple pruning method, coined lookahead pruning, by extending the single layer optimization to a multi-layer optimization. Our experimental results demonstrate that the proposed method consistently outperforms magnitude-based pruning on various networks, including VGG and ResNet, particularly in the high-sparsity regime. See https://github.com/alinlab/lookahead_pruning for codes.

==> app_nlp.tex <==
\section{Experiments on text classification}
In this section, we evaluate the performance of LAP on pruning recurrent neural networks. In particular, we prune the long short-term memory (LSTM, \citet{hochreiter1997long}) trained on xxx dataset \cite{xx} for the classification task. 


In the experiments, the ``sight range'' of LAP was fixed to the preceding and succeeding layers, instead of considering all recurrent connections into account.

We use the network consisting of the glove embedding of 50 dimension \cite{xx}, xx layers LSTMs with xx hidden dimension and linear layer after LSTM layers for the classification. We also restrict the number of tokens to 500 while we pad empty space to data containing less than 500 tokens. For training models, we utilize Adam optimizer with xx learning rate and train xx iterations for both pre-training and fine-tuning.



As in previous sections, we use magnitude-based pruning as a baseline.



==> commented.tex <==
\begin{comment}
\begin{table}[h]\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrrrrr|r}
\toprule
Rem. weights & 16.74\% & 14.23\% & 12.10\% & 10.28\% & 8.74\% & 7.43\%& 6.32\%& 5.37\%& 1.72\%\\
\midrule
MP (baseline) & 11.41{\scriptsize $\pm$0.24}& 11.72{\scriptsize $\pm$0.15}& 12.38{\scriptsize $\pm$0.14}& 12.64{\scriptsize $\pm$0.10}& 13.54{\scriptsize $\pm$0.35}& 14.84{\scriptsize $\pm$0.40}& 16.08{\scriptsize $\pm$1.13}& 17.23{\scriptsize $\pm$0.82}& 55.97{\scriptsize $\pm$15.99}\\
\midrule
LAP           & \textbf{11.19{\scriptsize $\pm$0.15}}& \textbf{11.45{\scriptsize $\pm$0.24}}& \textbf{11.79{\scriptsize $\pm$0.44}}& \textbf{11.93{\scriptsize $\pm$0.33}}& \textbf{12.95{\scriptsize $\pm$0.14}}& 13.42{\scriptsize $\pm$0.18}& \textbf{13.95{\scriptsize $\pm$0.17}}& \textbf{14.65{\scriptsize $\pm$0.48}}& 28.96{\scriptsize $\pm$3.30}\\
& \textbf{(-1.93\%)}& \textbf{(-2.30\%)}& \textbf{(-4.77\%)}& \textbf{(-5.62\%)}& \textbf{(-4.36\%)}& (-9.57\%)& \textbf{(-13.25\%)}& \textbf{(-14.97\%)}& (-48.26\%)\\
LAP-forward   & 11.47{\scriptsize $\pm$0.30}& 11.82{\scriptsize $\pm$0.15}& 12.33{\scriptsize $\pm$0.12}& 12.53{\scriptsize $\pm$0.19}& 13.15{\scriptsize $\pm$0.22}& \textbf{13.29{\scriptsize $\pm$0.14}}& 13.96{\scriptsize $\pm$0.25}& 14.67{\scriptsize $\pm$0.24}& \textbf{25.85{\scriptsize $\pm$1.40}}\\
& (+0.52\%)& (+0.85\%)& (-0.40\%)& (-0.87\%)& (-2.88\%)& \textbf{(-10.44\%)}& (-13.18\%)& (-14.86\%)& \textbf{(-53.81\%)}\\
\bottomrule
\end{tabular}}
\caption{Test error rates for VGG-11 at various sparsity levels. Subscripts denote the standard deviation over 5 trials, and bracketed numbers denote relative gain with respect to MP. The unpruned network achieved 11.51\% error rate.}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[h]\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrrrrr|r}
\toprule
Rem. weights & 16.74\% & 14.23\% & 12.10\% & 10.28\% & 8.74\% & 7.43\%& 6.32\%& 5.37\%& 1.72\%\\
\midrule
MP (baseline) & 11.41\%& 11.72\%& 12.38\%& 12.64\%& 13.54\%& 14.84\%& 16.08\%& 17.23\%& 55.97\%\\
& ($\pm$0.24)& ($\pm$0.15)& ($\pm$0.14)& ($\pm$0.10)& ($\pm$0.35)& ($\pm$0.40)& ($\pm$1.13)& ($\pm$0.82)& ($\pm$15.99)\\
\midrule
LAP           & \textbf{11.19\%}& \textbf{11.45\%}& \textbf{11.79\%}& \textbf{11.93\%}& \textbf{12.95\%}& 13.42\%& \textbf{13.95\%}& \textbf{14.65\%}& 28.96\%\\
& ($\pm$0.15)& ($\pm$0.24)& ($\pm$0.44)& ($\pm$0.33)& ($\pm$0.14)& ($\pm$0.18)& ($\pm$0.17)& ($\pm$0.48)& ($\pm$3.30)\\
LAP-forward   & 11.47\%& 11.82\%& 12.33\%& 12.53\%& 13.15\%& \textbf{13.29\%}& 13.96\%& 14.67\%& \textbf{25.85\%}\\
& ($\pm$0.30)& ($\pm$0.15)& ($\pm$0.12)& ($\pm$0.19)& ($\pm$0.22)& ($\pm$0.14)& ($\pm$0.25)& ($\pm$0.24)& ($\pm$1.40)\\
\bottomrule
\end{tabular}}
\caption{Test error rates for VGG-11 under various levels of sparsity. The unpruned network achieved 11.51\% error rate.}
\end{table}
\end{comment}
